Low-Rank Bandits via Tight Two-to-Infinity Singular Subspace Recovery

We study contextual bandits with low-rank structure where, in each round, if the (context, arm) pair $(i,j)\in [m]\times [n]$ is selected, the learner observes a noisy sample of the $(i,j)$-th entry of an unknown low-rank reward matrix. Successive contexts are generated randomly in an i.i.d. manner and are revealed to the learner. For such bandits, we present efficient algorithms for policy evaluation, best policy identification and regret minimization. For policy evaluation and best policy identification, we show that our algorithms are nearly minimax optimal. For instance, the number of samples required to return an $\varepsilon$-optimal policy with probability at least $1-\delta$ typically scales as ${r(m+n)\over \varepsilon^2}\log(1/\delta)$. Our regret minimization algorithm enjoys minimax guarantees typically scaling as $r^{7/4}(m+n)^{3/4}\sqrt{T}$, which improves over existing algorithms. All the proposed algorithms consist of two phases: they first leverage spectral methods to estimate the left and right singular subspaces of the low-rank reward matrix. We show that these estimates enjoy tight error guarantees in the two-to-infinity norm. This in turn allows us to reformulate our problems as a misspecified linear bandit problem with dimension roughly $r(m+n)$ and misspecification controlled by the subspace recovery error, as well as to design the second phase of our algorithms efficiently.

==> 4.subspacerecovery_old.tex <==
\section{Singular Subspace Recovery}\label{sec:subspacerecovery}

In the first phase of our algorithms for low-rank bandits, the singular subspaces of $M$ are estimated. In this section, we study the performance of this estimation procedure. We assume that the learner observes $T$ samples of noisy entries of $M$ chosen in an i.i.d. manner according to some distribution $\omega$ over $[m]\times [n]$, and that from these observations, she builds estimates of the singular subspaces of $M$. For simplicity, we assume that $\omega$ is known to the learner. This is without loss of generality in our settings\footnote{Indeed, we can estimate the context distribution $\rho$ using only $\widetilde{O}(1/\rho_{\min})$ samples, and select $j$ uniformly at random (refer to Appendix \ref{subsec:knowledge-of-context})}. We also assume that $\omega_{\min}=\min_{(i,j)\in [m]\times [n]}\omega_{i,j}>0$. 

%\red{S: Last sentence seem to be repetitive. Also: in maybe we should already in Assumption 1 introduce $\varrho>0$?}
 
\subsection{Subspace estimation}\label{subsec:subest} 
To estimate the singular subspaces of $M$, we construct $\widetilde{M}$ as: for all $(i,j)\in [m]\times [n]$,
\begin{align}
\label{eq:def_Mtilde_uniform}
    \widetilde{M}_{i,j} =  \frac{1}{T \omega_{i,j}} \sum_{t=1}^T (M_{i_t, j_t} + \xi_t) \indicator_{\lbrace (i_t, j_t) = (i,j)\rbrace}.
\end{align}
Then, we let $\widehat{M}$ be the best $r$-rank approximation of $\widetilde{M}$. More precisely, we write from the SVD of $\widetilde{M}$:
\begin{align}\label{eq:SVD_hat_M}
\widehat{M} = \widehat{U}\widehat{\Sigma} \widehat{V}^\top,    
\end{align}
where $\widehat{\Sigma}$ is the diagonal matrix containing the $r$ largest singular values of $\widetilde{M}$. $\widehat{U} \in \RR^{m\times r}$ contains their corresponding $r$ left singular vectors, and $\widehat{V} \in \RR^{n\times r}$ their corresponding $r$ right singular vectors. By Eckart-Young-Mirsky's theorem, the matrix $\widehat{M}$ is the best $r$-rank approximation of $\widetilde{M}$. We use $\widehat{U}$ and $\widehat{V}$ as our estimates of the singular subspaces spanned by $U$ and $V$, respectively.

In what follows, we denote by $\widehat{U}_{\perp} \in\RR^{m\times (m-r)}$ a matrix made of orthonormal vectors completing $\widehat{U}$ so as to obtain an orthonormal basis of $\mathbb{R}^m$. $\widehat{V}_\perp \in \RR^{n\times (n-r)}$ is constructed similarly.

\subsection{Guarantees in the two-to-infinity norm} 

% Studying the subspace recovery error in the two-to-infinity norm is technically involved. One of the state-of-the-art techniques to obtain such guarantees is the so-called leave-one-out argument (see \cite{chen2021spectral} and references therein). This argument cannot be applied directly when dealing with sequential decision making problems, because it heavily relies on the independence of the entries of the observed random matrix to be recovered. The argument can however be adapted to the case of dependent entries using Poisson approximation results \citep{stojanovic2024spectral}. Building on these ideas, we can establish the following theorem whose proof is sketched in appendix. 

%\textcolor{red}{S: we should be clearer that this is not really a novel result (refer to Theorem 1 in \cite{stojanovic2024spectral}), and our main contributions are in later sections.}

We wish to examine the performance of our subspace recovery method in the two-to-infinity norm. More precisely, we denote the left and right singular subspace recovery errors in this norm by 
\begin{align*}
    d_{2\to\infty}(U, \widehat{U}) = \Vert U U^\top - \widehat{U} \widehat{U}^\top \Vert_{2 \to \infty}, \\
    d_{2\to\infty}(V, \widehat{V}) = \Vert V V^\top - \widehat{V} \widehat{V}^\top \Vert_{2 \to \infty}.
\end{align*}
Now, we present the main guarantee on these errors, which is adapted from \cite{stojanovic2024spectral}.  
\begin{theorem}[Subspace recovery in $\Vert \cdot \Vert_{2 \to \infty}$]\label{thm:recovery-two-to-infinity-norm}
    Let us denote $\epsilon_{\textup{Sub-Rec}} := \max( d_{2\to\infty}(U,\widehat{U}), d_{2\to\infty}(V,\widehat{V}))$ and $L = \Vert M \Vert_{\max} \vee \sigma$. For any $\delta \in (0,1)$, the following event: 
%     \begin{align*}
%     \epsilon_{\textup{Sub-Rec}} \lesssim  \sqrt{\frac{\mu^6 \kappa^4 r^{3}  (m+n)}{T \omega_{\min} mn(m\wedge n)}\log^{3}\left( \frac{(m+n)T}{\delta}\right)}
% \end{align*}
%     holds with probability at least $1- \delta$, provided that
%     $$
%     T \gtrsim \frac{\mu^4 \kappa^2 r^2  (m+n)}{\omega_{\min} 
%  mn} \log^3\left( \frac{(m+n)T}{\delta}\right).
%     $$ 
    \begin{align*}
    \epsilon_{\textup{Sub-Rec}} \lesssim  \sqrt{\frac{L^2\kappa^2\mu^2 r (m+n) }{\sigma_r^2 T\omega_{\min}(m\wedge n)}\log^3\left(\frac{(m+n)T}{\delta}\right)}
    \end{align*}
    holds with probability at least $1- \delta$, provided that 
    \begin{align*}
    T \gtrsim \frac{L^2 (m+n)}{\sigma_r^2 \omega_{\min}} \log^3\left( \frac{(m+n)T}{\delta}\right).
    \end{align*}  
\end{theorem}

The proof of Theorem \ref{thm:recovery-two-to-infinity-norm} is sketched in Appendix \ref{sec:app_sing_sub_rec}. The analysis is technically involved and relies on combining the so-called leave-one-out argument (see \cite{chen2021spectral} and references therein) together with a Poisson approximation technique \cite{stojanovic2024spectral}. 




% To appreciate the statement of Theorem \ref{thm:recovery-two-to-infinity-norm}, it is instructive to apply the result in the case where the sampling distribution $p$ is the uniform distribution over $[m]\times[n]$. 

% \begin{corollary}[Recovery under uniform sampling] \label{cor:recovery-two-to-infinity-norm}
% Let $\delta \in (0, 1)$. Then, the following event
%     \begin{align*}
%     & \max\left(\Vert V V^\top - \widehat{V} \widehat{V}^\top \Vert_{2 \to \infty}, \Vert U U^\top - \widehat{U} \widehat{U}^\top\Vert_{2 \to \infty} \right)  \\ 
%     & \qquad \quad \le  C \mu^3 \kappa^2 r^{3/2} \sqrt{\frac{(m+n)}{T(m\wedge n)}\log^{3}\left( \frac{e(m+n)T}{\delta}\right)}, 
% \end{align*}
%  holds with probability at least $1- \delta$, provided that
%     $$
%     T \geq c \mu^4 \kappa^2 r^2(m+n) \log^3\left( \frac{e(m+n)T}{\delta}\right),
%     $$ for some universal constants $C,c>0$. 
% \end{corollary}

\textcolor{red}{S: need to add that $\sigma = O(\Vert M\Vert_{\max})$ for discussion below... Or we just say that Frobenius norm is $\sqrt{m+n}$ times larger...}
From Theorem \ref{thm:recovery-two-to-infinity-norm}, we see that if the matrix $M$ and the sampling distribution $\omega$ are homogeneous, then after only $\widetilde{\Omega}(m+n)$ observations, we can recover the singular subspaces with an error rate in the $\Vert \cdot \Vert_{2 \to \infty}$ norm that scales as $\widetilde{O}(1/\sqrt{T})$ with high probability. The recovery error in $\Vert \cdot \Vert_\F$ would typically scale as $\widetilde{O}(\sqrt{(m+n)/T})$ (see Lemma \ref{lemma:subspace_Frobenius}; it can also be established using classical arguments\footnote{By classical arguments, we mean using a matrix concentration bound such as matrix Bernstein inequality and Davis-Kahan-Wedin Theorem to obtain a high probability bound on $\Vert \widehat{V} \widehat{V}^\top - V V^\top \Vert_F$.} as in \cite{jun2019bilinear}). This suggests that the subspace recovery error (seen as a matrix) is {\it delocalized}, i.e., spread out along $m+n$ directions. Thus, the provided two-to-infinity norm guarantees offer a finer and more precise control over the subspace recovery error than the Frobenius norm guarantees. We take advantage of this when devising algorithms for contextual low-rank bandits. 



% This implies that the recovery error rate in Frobenius norm scales as $\widetilde{O}(\sqrt{(m+n)/T})$ (see Lemma \ref{lem:r}). This rate corresponds to the typical scaling under homogeneity and using classical arguments\footnote{By classical arguments, we mean using a matrix concentration bound such as matrix Bernstein inequality and Davis-Kahan-Wedin Theorem to obtain a high probability bound on $\Vert \widehat{V} \widehat{V}^\top - V V^\top \Vert_F$.} \cite{jun2019bilinear}. The guarantees provided  in Theorem \ref{thm:recovery-two-to-infinity-norm} are hence finer and stronger. 


%More importantly, our two-to-infinity guarantee is finer and stronger than traditionally considered guarantees in Frobenius norm. This constitutes a crucial observation towards the design of provably better algorithms for the envisioned learning tasks and will become apparent in the next sections.




% Studying the subspace recovery error in the two-to-infinity norm is technically involved. One of the state-of-the-art techniques to obtain such guarantees is the so-called leave-one-out argument (see \cite{chen2021spectral} and references therein). This argument cannot be applied directly when dealing with sequential decision making problems, because it heavily relies on the independence of the entries of the observed random matrix to be recovered. The argument can however be adapted to the case of dependent entries using Poisson approximation results \citep{stojanovic2024spectral}. Building on these ideas, we can establish the following theorem whose proof is sketched in appendix. 




% From Theorem \ref{thm:recovery-two-to-infinity-norm} in the case of uniform context distribution, \textcolor{red}{S: there are no contexts in Section 4, instead: "in the case of uniform sampling probabilities $p$"?} we observe that after only $\widetilde{\Omega}(m+n)$ observations, when $m+n = O(m \wedge n)$, we can recover the singular subspaces with an error rate in the $\Vert \cdot \Vert_{2 \to \infty}$ norm that is of order $\widetilde{O}(1/\sqrt{T})$ with high probability. 


